Shampoo: Preconditioned Stochastic Tensor Optimization

Preconditioned gradient methods are among the most general and powerful tools in optimization. However, preconditioning requires storing and manipulating prohibitively large matrices. We describe and analyze a new structure-aware preconditioning algorithm, called Shampoo, for stochastic optimization over tensor spaces. Shampoo maintains a set of preconditioning matrices, each of which operates on a single dimension, contracting over the remaining dimensions. We establish convergence guarantees in the stochastic convex setting, the proof of which builds upon matrix trace inequalities. Our experiments with state-of-the-art deep learning models show that Shampoo is capable of converging considerably faster than commonly used optimizers. Although it involves a more complex update rule, Shampoo's runtime per step is comparable to that of simple gradient methods such as SGD, AdaGrad, and Adam.

==> tensors.tex <==
\makeatletter

\newcommand{\tikzcuboid@shiftx}{0}
\newcommand{\tikzcuboid@shifty}{0}
\newcommand{\tikzcuboid@dimx}{3}
\newcommand{\tikzcuboid@dimy}{3}
\newcommand{\tikzcuboid@dimz}{3}
\newcommand{\tikzcuboid@scale}{1}
\newcommand{\tikzcuboid@densityx}{1}
\newcommand{\tikzcuboid@densityy}{1}
\newcommand{\tikzcuboid@densityz}{1}
\newcommand{\tikzcuboid@rotation}{0}
\newcommand{\tikzcuboid@anglex}{0}
\newcommand{\tikzcuboid@angley}{90}
\newcommand{\tikzcuboid@anglez}{225}
\newcommand{\tikzcuboid@scalex}{1}
\newcommand{\tikzcuboid@scaley}{1}
\newcommand{\tikzcuboid@scalez}{sqrt(0.5)}
\newcommand{\tikzcuboid@linefront}{black}
\newcommand{\tikzcuboid@linetop}{black}
\newcommand{\tikzcuboid@lineright}{black}
\newcommand{\tikzcuboid@fillfront}{white}
\newcommand{\tikzcuboid@filltop}{white}
\newcommand{\tikzcuboid@fillright}{white}
\newcommand{\tikzcuboid@shaded}{N}
\newcommand{\tikzcuboid@shadecolor}{black}
\newcommand{\tikzcuboid@shadeperc}{25}
\newcommand{\tikzcuboid@emphedge}{N}
\newcommand{\tikzcuboid@emphstyle}{thick}

% Definition of Keys
\define@key{tikzcuboid}{shiftx}[\tikzcuboid@shiftx]{\renewcommand{\tikzcuboid@shiftx}{#1}}
\define@key{tikzcuboid}{shifty}[\tikzcuboid@shifty]{\renewcommand{\tikzcuboid@shifty}{#1}}
\define@key{tikzcuboid}{dimx}[\tikzcuboid@dimx]{\renewcommand{\tikzcuboid@dimx}{#1}}
\define@key{tikzcuboid}{dimy}[\tikzcuboid@dimy]{\renewcommand{\tikzcuboid@dimy}{#1}}
\define@key{tikzcuboid}{dimz}[\tikzcuboid@dimz]{\renewcommand{\tikzcuboid@dimz}{#1}}
\define@key{tikzcuboid}{scale}[\tikzcuboid@scale]{\renewcommand{\tikzcuboid@scale}{#1}}
\define@key{tikzcuboid}{densityx}[\tikzcuboid@densityx]{\renewcommand{\tikzcuboid@densityx}{#1}}
\define@key{tikzcuboid}{densityy}[\tikzcuboid@densityy]{\renewcommand{\tikzcuboid@densityy}{#1}}
\define@key{tikzcuboid}{densityz}[\tikzcuboid@densityz]{\renewcommand{\tikzcuboid@densityz}{#1}}
\define@key{tikzcuboid}{rotation}[\tikzcuboid@rotation]{\renewcommand{\tikzcuboid@rotation}{#1}}
\define@key{tikzcuboid}{anglex}[\tikzcuboid@anglex]{\renewcommand{\tikzcuboid@anglex}{#1}}
\define@key{tikzcuboid}{angley}[\tikzcuboid@angley]{\renewcommand{\tikzcuboid@angley}{#1}}
\define@key{tikzcuboid}{anglez}[\tikzcuboid@anglez]{\renewcommand{\tikzcuboid@anglez}{#1}}
\define@key{tikzcuboid}{scalex}[\tikzcuboid@scalex]{\renewcommand{\tikzcuboid@scalex}{#1}}
\define@key{tikzcuboid}{scaley}[\tikzcuboid@scaley]{\renewcommand{\tikzcuboid@scaley}{#1}}
\define@key{tikzcuboid}{scalez}[\tikzcuboid@scalez]{\renewcommand{\tikzcuboid@scalez}{#1}}
\define@key{tikzcuboid}{linefront}[\tikzcuboid@linefront]{\renewcommand{\tikzcuboid@linefront}{#1}}
\define@key{tikzcuboid}{linetop}[\tikzcuboid@linetop]{\renewcommand{\tikzcuboid@linetop}{#1}}
\define@key{tikzcuboid}{lineright}[\tikzcuboid@lineright]{\renewcommand{\tikzcuboid@lineright}{#1}}
\define@key{tikzcuboid}{fillfront}[\tikzcuboid@fillfront]{\renewcommand{\tikzcuboid@fillfront}{#1}}
\define@key{tikzcuboid}{filltop}[\tikzcuboid@filltop]{\renewcommand{\tikzcuboid@filltop}{#1}}
\define@key{tikzcuboid}{fillright}[\tikzcuboid@fillright]{\renewcommand{\tikzcuboid@fillright}{#1}}
\define@key{tikzcuboid}{shaded}[\tikzcuboid@shaded]{\renewcommand{\tikzcuboid@shaded}{#1}}
\define@key{tikzcuboid}{shadecolor}[\tikzcuboid@shadecolor]{\renewcommand{\tikzcuboid@shadecolor}{#1}}
\define@key{tikzcuboid}{shadeperc}[\tikzcuboid@shadeperc]{\renewcommand{\tikzcuboid@shadeperc}{#1}}
\define@key{tikzcuboid}{emphedge}[\tikzcuboid@emphedge]{\renewcommand{\tikzcuboid@emphedge}{#1}}
\define@key{tikzcuboid}{emphstyle}[\tikzcuboid@emphstyle]{\renewcommand{\tikzcuboid@emphstyle}{#1}}

% Commands

\newcommand{\tikzvecx}[1]{
  \setkeys{tikzcuboid}{#1} % Process Keys passed to command
  \pgfmathsetmacro{\XDimx}{\tikzcuboid@dimx}
  \pgfmathsetmacro{\XDimy}{\tikzcuboid@dimy}
  \pgfmathsetmacro{\Steppingx}{1/\tikzcuboid@densityx}
  \pgfmathsetmacro{\Secondx}{2*\Steppingx}
  \pgfmathsetmacro{\Vectorxx}{\tikzcuboid@scalex*cos(\tikzcuboid@anglex)}
  \pgfmathsetmacro{\Vectorxy}{\tikzcuboid@scalex*sin(\tikzcuboid@anglex)}
  \pgfmathsetmacro{\Vectoryx}{\tikzcuboid@scaley*cos(\tikzcuboid@angley)}
  \pgfmathsetmacro{\Vectoryy}{\tikzcuboid@scaley*sin(\tikzcuboid@angley)}
  \begin{scope}[%
    xshift=\tikzcuboid@shiftx,%
    yshift=\tikzcuboid@shifty,%
    scale=\tikzcuboid@scale,%
    rotate=\tikzcuboid@rotation,%
    x={(\Vectorxx,\Vectorxy)},%
    y={(\Vectoryx,\Vectoryy)}]
  \pgfmathsetmacro{\lowy}{0}
  \pgfmathsetmacro{\y}{\Steppingx}
  \foreach \x in {\Steppingx,\Secondx,...,\XDimx} {
    \pgfmathsetmacro{\lowx}{(\x-\Steppingx)}
    \filldraw[fill=\tikzcuboid@fillfront,draw=\tikzcuboid@linefront]%
      (\lowx,\lowy) -- (\lowx,\y) -- (\x,\y) -- (\x,\lowy) -- cycle;
  }
  \draw[\tikzcuboid@emphstyle]%
    (0,\XDimy) -- (\XDimx,\XDimy) -- (\XDimx,\XDimy) -- (0,\XDimy) -- cycle;%
  \draw[\tikzcuboid@emphstyle]%
    (0,0) -- (0,\XDimy) -- (\XDimx,\XDimy) -- (\XDimx,0) -- cycle;%
  \draw[\tikzcuboid@emphstyle]%
    (\XDimx,0) -- (\XDimx,\XDimy) -- (\XDimx,\XDimy) -- (\XDimx,0) -- cycle;%
  \end{scope}
}

\newcommand{\tikzvecy}[1]{
  \setkeys{tikzcuboid}{#1} % Process Keys passed to command
  \pgfmathsetmacro{\Nimx}{\tikzcuboid@dimx}
  \pgfmathsetmacro{\Nimy}{\tikzcuboid@dimy}
  \pgfmathsetmacro{\Steppingy}{1/\tikzcuboid@densityy}
  \pgfmathsetmacro{\Secondy}{2*\Steppingy}
  \pgfmathsetmacro{\Vectorxx}{\tikzcuboid@scalex*cos(\tikzcuboid@anglex)}
  \pgfmathsetmacro{\Vectorxy}{\tikzcuboid@scalex*sin(\tikzcuboid@anglex)}
  \pgfmathsetmacro{\Vectoryx}{\tikzcuboid@scaley*cos(\tikzcuboid@angley)}
  \pgfmathsetmacro{\Vectoryy}{\tikzcuboid@scaley*sin(\tikzcuboid@angley)}
  \begin{scope}[%
    xshift=\tikzcuboid@shiftx,%
    yshift=\tikzcuboid@shifty,%
    scale=\tikzcuboid@scale,%
    rotate=\tikzcuboid@rotation,%
    x={(\Vectorxx,\Vectorxy)},%
    y={(\Vectoryx,\Vectoryy)}]
  \pgfmathsetmacro{\lowx}{0}
  \pgfmathsetmacro{\x}{\Steppingy}
  \foreach \y in {\Steppingy,\Secondy,...,\Nimy} {
    \pgfmathsetmacro{\lowy}{(\y-\Steppingy)}
    \filldraw[fill=\tikzcuboid@fillfront,draw=\tikzcuboid@linefront]%
      (\lowx,\lowy) -- (\lowx,\y) -- (\x,\y) -- (\x,\lowy) -- cycle;
  }
  \draw[\tikzcuboid@emphstyle]%
    (0,\Nimy) -- (\Nimx,\Nimy) -- (\Nimx,\Nimy) -- (0,\Nimy) -- cycle;%
  \draw[\tikzcuboid@emphstyle]%
    (0,0) -- (0,\Nimy) -- (\Nimx,\Nimy) -- (\Nimx,0) -- cycle;%
  \draw[\tikzcuboid@emphstyle]%
    (\Nimx,0) -- (\Nimx,\Nimy) -- (\Nimx,\Nimy) -- (\Nimx,0) -- cycle;%
  \end{scope}
}

\newcommand{\tikzcubone}[1]{
    \setkeys{tikzcuboid}{#1} % Process Keys passed to command
    \pgfmathsetmacro{\Vectorxx}{\tikzcuboid@scalex*cos(\tikzcuboid@anglex)}
    \pgfmathsetmacro{\Vectorxy}{\tikzcuboid@scalex*sin(\tikzcuboid@anglex)}
    \pgfmathsetmacro{\Vectoryx}{\tikzcuboid@scaley*cos(\tikzcuboid@angley)}
    \pgfmathsetmacro{\Vectoryy}{\tikzcuboid@scaley*sin(\tikzcuboid@angley)}
    \begin{scope}[xshift=\tikzcuboid@shiftx,%
      yshift=\tikzcuboid@shifty,%
      scale=\tikzcuboid@scale,%
      rotate=\tikzcuboid@rotation,%
      x={(\Vectorxx,\Vectorxy)},%
      y={(\Vectoryx,\Vectoryy)}]
  \pgfmathsetmacro{\Steppingx}{1/\tikzcuboid@densityx}
    \pgfmathsetmacro{\Steppingy}{1/\tikzcuboid@densityy}
    \newcommand{\Dimx}{\tikzcuboid@dimx}
    \newcommand{\Dimy}{\tikzcuboid@dimy}
    \pgfmathsetmacro{\Secondx}{2*\Steppingx}
    \pgfmathsetmacro{\Secondy}{2*\Steppingy}
    \foreach \x in {\Steppingx,\Secondx,...,\Dimx}
    {   \foreach \y in {\Steppingy,\Secondy,...,\Dimy}
        {   \pgfmathsetmacro{\lowx}{(\x-\Steppingx)}
            \pgfmathsetmacro{\lowy}{(\y-\Steppingy)}
            \filldraw[fill=\tikzcuboid@fillfront,draw=\tikzcuboid@linefront] (\lowx,\lowy) -- (\lowx,\y) -- (\x,\y) -- (\x,\lowy) -- cycle;
        }
    }
    \draw[\tikzcuboid@emphstyle](0,\Dimy) -- (\Dimx,\Dimy) -- (\Dimx,\Dimy) -- (0,\Dimy) -- cycle;%
    \draw[\tikzcuboid@emphstyle](0,0) -- (0,\Dimy) -- (\Dimx,\Dimy) -- (\Dimx,0) -- cycle;%
    \draw[\tikzcuboid@emphstyle](\Dimx,0) -- (\Dimx,\Dimy) -- (\Dimx,\Dimy) -- (\Dimx,0) -- cycle;%
    \end{scope}
}

\newcommand{\tikzcuboid}[1]{
    \setkeys{tikzcuboid}{#1} % Process Keys passed to command
    \pgfmathsetmacro{\vectorxx}{\tikzcuboid@scalex*cos(\tikzcuboid@anglex)}
    \pgfmathsetmacro{\vectorxy}{\tikzcuboid@scalex*sin(\tikzcuboid@anglex)}
    \pgfmathsetmacro{\vectoryx}{\tikzcuboid@scaley*cos(\tikzcuboid@angley)}
    \pgfmathsetmacro{\vectoryy}{\tikzcuboid@scaley*sin(\tikzcuboid@angley)}
    \pgfmathsetmacro{\vectorzx}{\tikzcuboid@scalez*cos(\tikzcuboid@anglez)}
    \pgfmathsetmacro{\vectorzy}{\tikzcuboid@scalez*sin(\tikzcuboid@anglez)}
    \begin{scope}[xshift=\tikzcuboid@shiftx, yshift=\tikzcuboid@shifty, scale=\tikzcuboid@scale, rotate=\tikzcuboid@rotation, x={(\vectorxx,\vectorxy)}, y={(\vectoryx,\vectoryy)}, z={(\vectorzx,\vectorzy)}]
    \pgfmathsetmacro{\steppingx}{1/\tikzcuboid@densityx}
    \pgfmathsetmacro{\steppingy}{1/\tikzcuboid@densityy}
    \pgfmathsetmacro{\steppingz}{1/\tikzcuboid@densityz}
    \newcommand{\dimx}{\tikzcuboid@dimx}
    \newcommand{\dimy}{\tikzcuboid@dimy}
    \newcommand{\dimz}{\tikzcuboid@dimz}
    \pgfmathsetmacro{\secondx}{2*\steppingx}
    \pgfmathsetmacro{\secondy}{2*\steppingy}
    \pgfmathsetmacro{\secondz}{2*\steppingz}
    \ifthenelse{\equal{\dimy}{0}}{}%
    {%
    \foreach \x in {\steppingx,\secondx,...,\dimx}%
    {   \foreach \y in {\steppingy,\secondy,...,\dimy}%
        {   \pgfmathsetmacro{\lowx}{(\x-\steppingx)}%
            \pgfmathsetmacro{\lowy}{(\y-\steppingy)}%
            \filldraw[fill=\tikzcuboid@fillfront,draw=\tikzcuboid@linefront] (\lowx,\lowy,\dimz) -- (\lowx,\y,\dimz) -- (\x,\y,\dimz) -- (\x,\lowy,\dimz) -- cycle;% 
        }%
    }%
    }
    \ifthenelse{\equal{\dimx}{0}}{}%
    {%
    \foreach \x in {\steppingx,\secondx,...,\dimx}%
    {   \foreach \z in {\steppingz,\secondz,...,\dimz}%
        {   \pgfmathsetmacro{\lowx}{(\x-\steppingx)}%
            \pgfmathsetmacro{\lowz}{(\z-\steppingz)}%
            \filldraw[fill=\tikzcuboid@filltop,draw=\tikzcuboid@linetop] (\lowx,\dimy,\lowz) -- (\lowx,\dimy,\z) -- (\x,\dimy,\z) -- (\x,\dimy,\lowz) -- cycle;%
        }%
    }%
    }
    \ifthenelse{\equal{\dimy}{0}}{}%
    {%
    \foreach \y in {\steppingy,\secondy,...,\dimy}%
    {   \foreach \z in {\steppingz,\secondz,...,\dimz}%
        {   \pgfmathsetmacro{\lowy}{(\y-\steppingy)}%
            \pgfmathsetmacro{\lowz}{(\z-\steppingz)}%
            \filldraw[fill=\tikzcuboid@fillright,draw=\tikzcuboid@lineright] (\dimx,\lowy,\lowz) -- (\dimx,\lowy,\z) -- (\dimx,\y,\z) -- (\dimx,\y,\lowz) -- cycle;%
        }%
    }%
    }
    \ifthenelse{\equal{\tikzcuboid@emphedge}{Y}}%
        {\draw[\tikzcuboid@emphstyle](0,\dimy,0) -- (\dimx,\dimy,0) -- (\dimx,\dimy,\dimz) -- (0,\dimy,\dimz) -- cycle;%
        \draw[\tikzcuboid@emphstyle] (0,0,\dimz) -- (0,\dimy,\dimz) -- (\dimx,\dimy,\dimz) -- (\dimx,0,\dimz) -- cycle;%
        \draw[\tikzcuboid@emphstyle](\dimx,0,0) -- (\dimx,\dimy,0) -- (\dimx,\dimy,\dimz) -- (\dimx,0,\dimz) -- cycle;%
        }%
        {}
    \end{scope}
}

\makeatother

